Budget-Constrained Step-Level Diffusion Caching

Step-level caching accelerates diffusion models by exploiting temporal redundancy across denoising steps. Existing methods make per-step cache decisions using threshold-based heuristics, without directly optimizing for final output quality. As a result, their inference latency varies across inputs and is difficult to control at deployment. In this work, we propose BudCache, which inverts this formulation: rather than letting per-step error thresholds dictate the runtime cost, we fix the compute budget in advance and search for the cache policy that best preserves the final output. To tackle the combinatorial complexity of step selection, we combine Simulated Annealing with deterministic Hill Climbing. This offline search identifies high-quality cache policies within minutes and introduces no online search or thresholding overhead during inference. When the compute budget is very tight, we further introduce cache-aware schedule alignment, which adapts the time discretization to the selected cache policy to reduce cache-induced trajectory mismatch. Experiments on FLUX.1-dev and Wan2.1 show that BudCache achieves better generation quality than heuristic caching baselines under the same inference budgets. Code is available at https://github.com/Westlake-AGI-Lab/BudCache

==> figs/cap_nfesearchspace.tex <==
\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=.9\linewidth]{figs/nfeSearchSpace.pdf}}
\caption{
\textbf{ Impact of Search Space Size under Fixed Computational Budget (10 NFE)}.
We evaluate generation quality across different total inference step configurations ($T \in [15, 50]$) while maintaining a strict budget of 10 function evaluations.
All metrics exhibit a consistent \textbf{inverted-U trajectory}.
Quality initially improves as the total steps increase, benefiting from a more refined scheduler trajectory. However, performance degrades beyond Step 30 due to error accumulation from aggressive caching ratios.
}
\label{fig:nfesearchspace}
\end{center}
\end{figure}
